A Model-Based Approach for Specifying Changes in Replications of Empirical Studies in Computer Science

Context: The need of replicating empirical studies in Computer Science (CS) is widely recognized among the research community to consolidate acquired knowledge generalizing results. It is essential to report the changes of each replication to understand the evolution of the experimental validity across a family of studies. Unfortunately, the lack of proposals undermines these objectives. Objective. The main goal of our work is to provide researchers in CS, and in other areas of research, with a systematic, tool-supported approach for the reporting of changes in the replications of their empirical studies. Method: Applying DSR, we have developed and validated a composite artifact consisting of (i) a metamodel of the relevant concepts of replications and their changes; (ii) templates and linguistic patterns for reporting those concepts; and (iii) a proof-of-concept model-based software tool that supports the proposed approach. For its validation, we have carried out a multiple case study including 9 families of empirical studies from CS and Agrobiology. The 9 families encompass 23 replication studies and 92 replication changes, for which we have analyzed the suitability of our proposal. Results: The multiple case study revealed some initial limitations of our approach related to threats to experimental validity or context variables. After several improvement iterations, all the 92 replication changes could be properly specified, including also their qualitatively estimated effects on experimental validity across the family of experiments and its corresponding visualization. Conclusions: Our proposal for the specification of replication changes seems to fit the needs not only of replications in CS, but also in other research areas. Nevertheless, further research is needed to improve it and to disseminate its use among the research community.

==> figures/T-DSR.tex <==
% ----------------------------
% File    : T-DSR.tex
% Content : Tabla DRS
% Date    : 1/12/2018
% Version : 1.0
% Authors : M.Cruz
% ----------------------------
\begin{table*}
  \caption{Activities of the \DSR methodology and corresponding sections}
  \label{tab:fases-DSR}
  \centering
%   \footnotesize \footnotesize
  \begin{tabularx}{0.98\textwidth}{
      >{\hsize=0.3\hsize}X
      >{\hsize=0.6\hsize}X
      >{\hsize=0.1\hsize}c}

 
    \toprule
    Actividad  &
    Descripción   &
    Sección \\
    \midrule
    
    \emph{Problem identification and motivation}  &
    Need to address an accurate definition of changes for the reporting of replications of controlled experiments & 
    \ref{sec:intro}  \\ 
    
    \emph{Solution objectives definition}  & 
    Facilitate documentation of changes so that they are clearly specified.  The information involved in the changes is analysed and other proposals are identified &
    \ref{sec:background}, \ref{sec:metamodelo} \\
    
    \emph{Design and Development}  & 
    A meta--model is proposed. A possible implementation of the meta--model is the template completed with L-patterns & 
    \ref{sec:metamodelo}, \ref{sec:plantilla} \\
    
    \emph{Demonstration}  &
    The first version of the template is instantiated by defining the changes of a family of experiments belonging to the \gls{SE} area  &
    \ref{sec:case_study} \\
    
    \emph{Evaluation}  &
    The artefact, in our case the template, is evaluated in a multiple case study encompassing various areas of knowledge and types of experiments. CÆSAR tool is used as a proof of concept & 
    \ref{sec:case_study} \\
    
    \emph{Communication} & 
    The results of the research are published &  \\ 
    
    \bottomrule
  	\end{tabularx}   
\end{table*}

==> figures/T-Nomenclature.tex <==
% -----------------------------------
% File    : T-Nomenclature.tex
% Content : Compara la nomenclatura 
% Date    : 7/Mayo/2019
% Version : 1.0
% Authors : M.Cruz
% -----------------------------------

% -----------------------------------
% Last update: 4/04/2020 (MCruz)
% Actualización a partir de la tesis
% -----------------------------------

\begin{table}[htbp]
 
\caption{Comparison of nomenclature used in \SoftEng-Case, \Science-Case and \Automatic-Case}
    \label{tab:T-Nomencla}
    \centering

    \begin{tabularx}{0.95\textwidth}{Xcc}
    \toprule
   
\SoftEng-Case &  
\Science-Case & 
\Automatic-Case  \\

\noalign{\smallskip}\hline\noalign{\smallskip}
	Replication             & 
	Repetition with changes & 
	Replication             \\
	
	Repetition & 
	Repetition & 
	Repetition \\
	
	Reproduction & 
	\ding{55}    & 
	Reproduction \\
	
	Replication type & 
	\ding{55}        & 
	Replication type \\
	
	Family experiments & 
	\ding{55}          & 
	\ding{55}          \\
	
\noalign{\smallskip}\hline\noalign{\smallskip}
    Dependent variable$^1$ & 
    Dependent variable & 
    Dependent variable \\
    
    Independent variable$^2$ & 
    Independent variable &  Independent variable \\
    
    Context variable & 
    \ding{55} & 
    Context variable \\
    
    Blocking variable &
    Blocking variable &
    Blocking variable \\
    
    Parameters & 
    Parameters & 
    Parameters \\

    Level & 
    Level &
    Level \\
  
\noalign{\smallskip}\hline\noalign{\smallskip}

    Experimental subject & 
    Experimental subject &
    \ding{55}            \\
    
    Experimental object$^3$ & 
    Experimental unit       &  
    Experimental unit       \\
    
    Population & 
    Population & 
    Population \\

\noalign{\smallskip}\hline\noalign{\smallskip}
	
    Threats to validity & 
    \ding{55}           & 
    Threats to validity \\
    
    Internal validity & 
    \ding{55}         & 
    Internal validity \\
    
    External validity & 
    \ding{55}         & 
    External validity \\
    
    Construct validity & 
    \ding{55}          & 
    Construct validity \\
    
    Conclusion validity & 
    \ding{55} & 
    Conclusion validity \\
    
\noalign{\smallskip}\hline\noalign{\smallskip}

    Experimental design & 
    Experimental design & 
    Experimental design \\
    
    Modified dimension & 
    \ding{55}          &
    \ding{55}          \\
    
    Operationalization & 
    \ding{55}          & 
    \ding{55}          \\
    
    Protocol$^4$ & 
    Procedure    & 
    Protocol     \\
    
    Treatment & 
    Treatment & 
    Treatment \\
    
    Guides & 
    Guides & 
    Guides \\

    \bottomrule
  
\multicolumn{3}{l}{$^1$ Also called response variable}   \\ 
\multicolumn{3}{l}{$^2$ Also called factor}   \\ 
\multicolumn{3}{l}{$^3$ Also called experimental unit}   \\ 
\multicolumn{3}{l}{$^4$ Also called experimental procedure}   \\
	  
\end{tabularx}  
\end{table}

==> figures/T-SC-Nomenclature.tex <==
% -----------------------------------
% File    : T-Nomenclature.tex
% Content : Compara la nomenclatura 
% Date    : 7/Mayo/2019
% Version : 1.0
% Authors : M.Cruz
% -----------------------------------

% -----------------------------------
% Last update: 4/04/2020 (MCruz)
% Actualización a partir de la tesis
% -----------------------------------

\begin{table*}[htbp]
 
\caption{Comparison of nomenclature used in \SoftEng-Case, \Science-Case and \Automatic-Case}
    \label{tab:T-Nomencla}
    \centering

    \begin{tabularx}{0.95\textwidth}{Xcc}
    \toprule
   
\SoftEng-Case &  
\Science-Case & 
\Automatic-Case  \\

\noalign{\smallskip}\hline\noalign{\smallskip}
	Replication             & 
	Repetition with changes & 
	Replication             \\
	
	Repetition & 
	Repetition & 
	Repetition \\
	
	Reproduction & 
	\ding{55}    & 
	Reproduction \\
	
	Replication type & 
	\ding{55}        & 
	Replication type \\
	
	Family experiments & 
	\ding{55}          & 
	\ding{55}          \\
	
\noalign{\smallskip}\hline\noalign{\smallskip}
    Dependent variable & 
    Dependent variable & 
    Dependent variable \\
    
    Independent variable$^1$ & 
    Independent variable$^1$ &  Independent variable$^1$ \\
    
    Context variable & 
    \ding{55} & 
    Context variable \\
    
    Blocking variable &
    Blocking variable &
    Blocking variable \\
    
    Parameters & 
    Parameters & 
    Parameters \\

    Level & 
    Level &
    Level \\
  
\noalign{\smallskip}\hline\noalign{\smallskip}

    Experimental subject & 
    Experimental subject &
    \ding{55}            \\
    
    Experimental object$^2$ & 
    Experimental unit       &  
    Experimental unit       \\
    
    Population & 
    Population & 
    Population \\

\noalign{\smallskip}\hline\noalign{\smallskip}
	
    Threats to validity & 
    \ding{55}           & 
    Threats to validity \\
    
    Internal validity & 
    \ding{55}         & 
    Internal validity \\
    
    External validity & 
    \ding{55}         & 
    External validity \\
    
    Construct validity & 
    \ding{55}          & 
    Construct validity \\
    
    Conclusion validity & 
    \ding{55} & 
    Conclusion validity \\
    
\noalign{\smallskip}\hline\noalign{\smallskip}

    Experimental design & 
    Experimental design & 
    Experimental design \\
    
    Modified dimension & 
    \ding{55}          &
    \ding{55}          \\
    
    Operationalization & 
    \ding{55}          & 
    \ding{55}          \\
    
    Protocol$^3$ & 
    Procedure    & 
    Protocol     \\
    
    Treatment & 
    Treatment & 
    Treatment \\
    
    Guides & 
    Guides & 
    Guides \\

    \bottomrule
  
\multicolumn{3}{l}{$^1$ También se denomina factor}   \\ 
\multicolumn{3}{l}{$^2$ También se denomina unidad experimental  \cite{Juristo}}   \\ 
\multicolumn{3}{l}{$^3$ También se denomina procedimiento experimental}   \\
	  
\end{tabularx}  
\end{table*}


==> figures/T-SC-Template-Soil.tex <==
% ------------------------------------------------------
% File    : T-NS-Soil.tex 
% Content : Replication Soil-2018 (Carmen2018.tex)
% Date    : 2/4/2019
% Version : 1.0
% Authors : C.Florido and M.Cruz
% ------------------------------------------------------
\begin{table*}[h]
    \caption{Specification of the first 5 changes of Soil-2018 replication using the template}
  
    \label{tab:template-Soil}
    \centering
	\scriptsize

    \begin{tabularx}{\textwidth}{
        >{\hsize=0.15\hsize}X
        >{\hsize=0.85\hsize}X}
  
    \toprule

    Replication & 
    \textbf{\emph{Soil-2018}}   Internal replication based on \textbf{\emph{Soil-2016}} original experiment  \\
	
	\midrule   
     
    Goal of experiment & 
        To evaluate the effect of a bio-surfactant on the assisted phytoremediation of contaminated soil \\  
        
    Description  & Whether the addition of the biosurfactant JBR-425 to two types of copper (Cu) contaminated soils (cause) reduces the Cu concentration in these soils is analysed by determining the Cu extracted (effect) by barley (\emph{Hordeum vulgare}) and mustard (\emph{Brassica juncea}) plants germinated in these soils.\\    
 
    Site and Date & 
        The base experiment was carried out in  \textit{Instituto de Recursos Naturales y Agrobiología de Sevilla (IRNAS)}  in  \textit{October 2016} \\ & 
        and this replication, in  \textit{Escuela Técnica Superior de Ingeniería Agronómica (ETSIA)-University of Seville} in \textit{March 2018} \\
    
    Purpose  &  
        Generalise results  Overcome some limitations of the  baseline experiment \\
%        Generalise results \\
%       &  Overcome some limitations of the  baseline experiment \\

\hline   
%-------------------------- 
    Change \textit{1}   &
        \textbf{Growing medium} \\ &
        \textbf{Originally}, the experiment was carried out in a cultivation chamber. \\& \textbf{In replication}, was carried out in a greenhouse \\& \textbf{In order to} simulate natural conditions \\
    
    Modified Dimension & 
        \textbf{Context}, specifically,
        the Growing medium of experimental unit \\
    
    Threat to validity  & 
        The change increases the external validity 
        since it allows to generalise the results carrying out the replication in conditions closer to natural ones \\  

\hline
%-------------------------- 
    Change \textit{2}   & 
        \textbf{Plant types} \\ &
        \textbf{Originally}, two plants were used: \emph{Hordeum vulgare} and \emph{Brassica juncea} \\& \textbf{In replication}, only \emph{Brassica juncea} was used \\& \textbf{Because} in the original experiment it was demonstrated that only \emph{Brassica juncea} was a metal accumulator plant\\  

    Modified Dimension & 
        \textbf{Protocol}, specifically measuring instruments \\   
        
    Threat to validity  & 
        The change increases construct validity due the effect can be measured in the mustard (\emph{Brassica juncea}), i.e. the extracted Cu  \\  
        
\hline
%-------------------------- 
    Change \textit{3}   & 
        \textbf{Soil types}  \\ &
        \textbf{Originally}, there were two types of soil: Coria (pH=7.8) and Constantina (pH=5.5) \\& \textbf{In replication}, only Constantina soil was used \\& \textbf{Because} it was demonstrated that in the soil of Coria the metal was strongly adsorbed and the phytoextraction did not affect the biomass production   \\  
    Modified Dimension & 
        \textbf{Population}, specifically the type of soil \\   
    
    Threat to validity  & 
        The change increases the construct validity since it ensures that the metal can be extracted from the soil. The extracted Cu is the effect to be measured. \\  
        
\hline
%-------------------------- 
    Change \textit{4}   & 
        \textbf{Copper dose reduction} \\ &
        \textbf{Originally}, Copper (Cu) doses were 0, 500 and 1000 mg $kg^{-1}$ \\& \textbf{In replication}, Cu doses were adjusted to 0, 125, 250 and 500 mg $kg^{-1}$     \\ 
        & \textbf{Because of} Cu doses of 1000 mg $kg^{-1}$ was toxic to the plant \\  
 
    Modified Dimension & 
        \textbf{Operationalization}, specifically the cause \\
        
    Threat to validity & 
        The change increases construct validity because the Cu dose is adjusted to non-toxic levels for the plant \\ 
        & The change increases internal validity because the effect is analysed at valid Cu levels \\

\hline
%-------------------------- 
    Change \textit{5}   & 
        \textbf{Form of application of copper} \\ &
        \textbf{Originally}, Cu was applied as Copper Nitrate \\& \textbf{In replication}, Cu was applied as Copper Sulfate \\
        & \textbf{Because of} is more accessible and the concentrations applied do not affect the plant \\  
 
    Modified Dimension & 
        \textbf{Operationalization}, specifically the cause \\
        
    Threat to validity  & 
        The change does not affect validity because the reactive is equivalent. \\  
 
\bottomrule
%	\noalign{\smallskip\smallskip}\hline
	\end{tabularx}  

\end{table*}


==> figures/caesar_changes.tex <==
% ----------------------------------------
% File    : caesar_changes.tex
% Content : Screenshots of CAESAR changes
% Date    : 15/05/2021
% Version : 1.0
% Authors : Amador
% ----------------------------------------

% ------------------------------------------
% Last update: 15/5/2021 (Amador)
% First version. The minipage is the only way
% to keep the three screenshots together.
% It requires the caption package.
% ------------------------------------------

\begin{figure}[h!]
  \begin{minipage}[c]{\columnwidth}
    \centering
    % trim = {left bottom right top}
    \includegraphics[scale=0.525,trim={0.275cm 0cm 0.25cm 0.15cm},clip]
    {figures/caesar_mind_2_change_2.png}
    \captionof{figure}{Specification of the second change of the \case{MIND\#2} replication}
    \label{fig:caesar-mind_2_2}

    % trim = {left bottom right top}
    \includegraphics[scale=0.525,trim={0cm 1.45cm 0cm 2.0cm},clip]
    {figures/caesar_mind_2_change_3.png}
    \captionof{figure}{Specification of the third change of the \case{MIND\#2} replication}
    \label{fig:caesar-mind_2_3}

    % trim = {left bottom right top}
    \includegraphics[scale=0.525,trim={0cm 1.4cm 0cm 2.0cm},clip]
    {figures/caesar_soil_2018_change_4.png}
    \captionof{figure}{Specification of the fourth change of the \case{Soil--2018} replication}
    \label{fig:caesar-soil_2018_4}
  \end{minipage}
\end{figure}

